Knowledge of Pretrained Language Models on Surface Information of Tokens

Do pretrained language models have knowledge regarding the surface information of tokens? We examined the surface information stored in word or subword embeddings acquired by pretrained language models from the perspectives of token length, substrings, and token constitution. Additionally, we evaluated the ability of models to generate knowledge regarding token surfaces. We focused on 12 pretrained language models that were mainly trained on English and Japanese corpora. Experimental results demonstrate that pretrained language models have knowledge regarding token length and substrings but not token constitution. Additionally, the results imply that there is a bottleneck on the decoder side in terms of effectively utilizing acquired knowledge.

==> tables/intro_table.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|l}
\hline
I      & How many letters is ``anthropologist''?  \\ 
O & The word ``anthropologist'' has 13 letters. \\ \hline
I      & What is the seventh letter of ``anthropologist''? \\ 
O & The seventh letter of ``anthropologist'' is ``o.'' \\\hline
I      & \cjk{「人類学者」は何文字の単語ですか？} \\ 
O & \cjk{「人類学者」は日本語で5文字の単語です。} \\\hline
I      & \cjk{「人類学者」の3文字目は何ですか？} \\ 
O & \cjk{「人類学者」の3文字目は「者」です。} \\\hline
\end{tabular}
\caption{
    Input (I) and output (O) examples for the case where asking surface information of wors to GPT-3.5 (as of 1st, Jan. 2024).
    The Japanese example means the same as the English texts, which asking the length and the third character in \cjk{人類学者} (anthropologist).
    \label{tbl:intro_table}
}
\end{table}



